A Survey of Efficient Reasoning for Large Reasoning Models: Language, Multimodality, and Beyond

Recent Large Reasoning Models (LRMs), such as DeepSeek-R1 and OpenAI o1, have demonstrated strong performance gains by scaling up the length of Chain-of-Thought (CoT) reasoning during inference. However, a growing concern lies in their tendency to produce excessively long reasoning traces, which are often filled with redundant content (e.g., repeated definitions), over-analysis of simple problems, and superficial exploration of multiple reasoning paths for harder tasks. This inefficiency introduces significant challenges for training, inference, and real-world deployment (e.g., in agent-based systems), where token economy is critical. In this survey, we provide a comprehensive overview of recent efforts aimed at improving reasoning efficiency in LRMs, with a particular focus on the unique challenges that arise in this new paradigm. We identify common patterns of inefficiency, examine methods proposed across the LRM lifecycle, i.e., from pretraining to inference, and discuss promising future directions for research. To support ongoing development, we also maintain a real-time GitHub repository tracking recent progress in the field. We hope this survey serves as a foundation for further exploration and inspires innovation in this rapidly evolving area.

==> summary.tex <==
\begin{table*}[!t]
\centering
\caption{Summary of Macro Action method. \textbf{Tag}: \encircle[fill=harvestgold, text=white]{I} = \underline{I}mage, \encircle[fill=lightcoral, text=white]{T} = \underline{T}ext, \encircle[fill=DarkGreen, text=white]{V} = \underline{V}ideo. Action Category: AD: Analysis and Decomposition, IPR: Information Processing and Reasoning, VC: Verification and Correction, GO: Generation and Optimization, EB: Exploration and Backtracking.}  

\resizebox{0.98\textwidth}{!}{
   \begin{tabular}% 
   {lllllccc}
    \toprule
        \multirow{2}{*}{\textbf{Methods}} & \multirow{2}{*}{\textbf{Usage}} & \multicolumn{5}{c}{\textbf{Action Attribute}} & \multirow{2}{*}{\textbf{Main Action Category}} \\ \cline{3-7}
          & & \textbf{Action Source} & \textbf{Action Number} & \textbf{Learning} & \textbf{Reflection} & \textbf{Modality} & \\ \midrule
        % RLHF
       \rowcolor[rgb]{ .949,  .949,  .949} Self-Check\cite{miao2023selfcheck} & Verification & Human-Designed & 4 & ICL & \textcolor{green}{\ding{51}} & \encircle[fill=lightcoral, text=white]{T} & AD, VC \\
       
        LeMa\cite{LeMa} & Synthetic Data & Human-Designed & 3 & ICL \& SFT & \textcolor{green}{\ding{51}} & \encircle[fill=lightcoral, text=white]{T} & VC, IPR \\
        
       \rowcolor[rgb]{ .949,  .949,  .949} REFINER\cite{li2024refiner} & Verification/Exploration & Human-Designed & 2 & ICL \& SFT & \textcolor{green}{\ding{51}} & \encircle[fill=lightcoral, text=white]{T} & VC, AD \\
        
        HiICL-MCTS\cite{HiICL-MCTS} & Exploration & Human-Designed & 5 & ICL & \textcolor{green}{\ding{51}} & \encircle[fill=lightcoral, text=white]{T} & VC, EB, AD  \\
        
         \rowcolor[rgb]{ .949,  .949,  .949} SUPERCORRECT\cite{yang2024supercorrect} & Distill & In-Context Learning & Dynamic & SFT \& RL & \textcolor{red}{\ding{55}} & \encircle[fill=lightcoral, text=white]{T} & AD, IPR \\
        
        ReasonFlux\cite{ReasonFlux}  & Synthetic Data/Exploration & Human-Designed & $\sim$500 & ICL \& SFT \& RL & \textcolor{red}{\ding{55}} &  \encircle[fill=lightcoral, text=white]{T} & AD, IPR \\
        
         \rowcolor[rgb]{ .949,  .949,  .949} rStar\cite{rSTaR} & Exploration & Human-Designed & 5 & ICL \& RL & \textcolor{green}{\ding{51}} & \encircle[fill=lightcoral, text=white]{T} & VC, GO, EB \\
         
        LLaMA-Berry\cite{zhang2024llama} & Exploration & Human-Designed & 2 & ICL \& RL & \textcolor{green}{\ding{51}} & \encircle[fill=lightcoral, text=white]{T} & VC, EB \\
    
        \rowcolor[rgb]{ .949,  .949,  .949} Huatuo-o1\cite{Huatuo-o1} & Synthetic Data & Human-Designed & 4 & ICL \& SFT & \textcolor{green}{\ding{51}} & \encircle[fill=lightcoral, text=white]{T} & VC \\

        Marco-o1\cite{Marco_o1} & Verification & Human-Designed & 1 & ICL \& SFT & \textcolor{green}{\ding{51}} & \encircle[fill=lightcoral, text=white]{T} & VC \\
        
         \rowcolor[rgb]{ .949,  .949,  .949}BoT\cite{yang2024buffer} & Exploration & In-Context Learning & Dynamic & ICL & \textcolor{red}{\ding{55}} & \encircle[fill=lightcoral, text=white]{T} & AD, IPR \\
         
        rStar-Math\cite{guan2025rstarmathsmallllmsmaster} & Exploration &  In-Context Learning & $1$ & ICL \& RL & \textcolor{green}{\ding{51}} & \encircle[fill=lightcoral, text=white]{T} & AD, IPR \\
        
         \rowcolor[rgb]{ .949,  .949,  .949}Mulberry\cite{yao2024mulberry} & Synthetic Data & In-Context Learning & 1 & ICL \& SFT & \textcolor{green}{\ding{51}}  & \encircle[fill=lightcoral, text=white]{T} & VC, EB \\
         
        LLaVA-CoT\cite{xu2024llava} & Synthetic Data/Exploration & Human-Designed & 4 & SFT & \textcolor{red}{\ding{55}} & \encircle[fill=harvestgold, text=white]{I} \space \encircle[fill=lightcoral, text=white]{T} & AD, IPR \\
        
         \rowcolor[rgb]{ .949,  .949,  .949}LLaMAV-o1\cite{thawakar2025llamav} & Verification/Exploration & Human-Designed & 4173 & Curriculum Learning & \textcolor{green}{\ding{51}} &  \encircle[fill=harvestgold, text=white]{I} \space \encircle[fill=lightcoral, text=white]{T} & AD, IPR \\
         
        AtomThink\cite{atomthink} & Synthetic Data/Exploration & In-Context Learning & $>$100 & SFT \& RL & \textcolor{green}{\ding{51}} & \encircle[fill=harvestgold, text=white]{I} \space \encircle[fill=lightcoral, text=white]{T} & AD, IPR, EB \\

         \rowcolor[rgb]{ .949,  .949,  .949}RedStar\cite{RedStar} & Distill & Human-Designed & 2 & SFT & \textcolor{green}{\ding{51}} & \encircle[fill=harvestgold, text=white]{I} \space \encircle[fill=lightcoral, text=white]{T} & AD, VC \\
        
        Auto-CoT \cite{zhangautomatic}  & Exploration & In-Context Learning & 2 & ICL & \textcolor{red}{\ding{55}} & \encircle[fill=lightcoral, text=white]{T} & AD, IPR, GO \\
        
         \rowcolor[rgb]{ .949,  .949,  .949}PoT\cite{chen2022program} & Verification & In-Context Learning & 1 & ICL & \textcolor{red}{\ding{55}} & \encircle[fill=lightcoral, text=white]{T} & AD, IPR, GO \\
        
        PAL\cite{gao2023pal} & Verification & In-Context Learning & 1 & ICL & \textcolor{red}{\ding{55}} & \encircle[fill=lightcoral, text=white]{T} & AD, IPR, GO \\
        
         \rowcolor[rgb]{ .949,  .949,  .949} Decomposed Prompt\cite{decomposed} & Exploration & Human-Designed & 3 & ICL & \textcolor{red}{\ding{55}} & \encircle[fill=lightcoral, text=white]{T} & AD, IPR \\
        
        Least-to-Most\cite{least2most} & Exploration & Human-Designed & 2 & ICL & \textcolor{red}{\ding{55}} & \encircle[fill=lightcoral, text=white]{T} & AD, IPR \\
        \bottomrule
   \end{tabular}
}
    \label{table:macro_action}
\end{table*}
